IoT-KEEPER: Securing IoT Communications in Edge Networks

The increased popularity of IoT devices have made them lucrative targets for attackers. Due to insecure product development practices, these devices are often vulnerable even to very trivial attacks and can be easily compromised. Due to the sheer number and heterogeneity of IoT devices, it is not possible to secure the IoT ecosystem using traditional endpoint and network security solutions. To address the challenges and requirements of securing IoT devices in edge networks, we present IoT-Keeper, which is a novel system capable of securing the network against any malicious activity, in real time. The proposed system uses a lightweight anomaly detection technique, to secure both device-to-device and device-to-infrastructure communications, while using limited resources available on the gateway. It uses unlabeled network data to distinguish between benign and malicious traffic patterns observed in the network. A detailed evaluation, done with real world testbed, shows that IoT-Keeper detects any device generating malicious traffic with high accuracy (0.982) and low false positive rate (0.01). The results demonstrate that IoT-Keeper is lightweight, responsive and can effectively handle complex D2D interactions without requiring explicit attack signatures or sophisticated hardware.

==> sections/challenges.tex <==
%!TEX root = ../iotguard.tex
Conventional network and endpoint security solutions fall short in addressing the challenges raised by IoT ecosystem, for a number of reasons:

\subsubsection*{\textbf{Heterogeneity of Ecosystem}}
The emerging IoT ecosystem consists of numerous heterogeneous devices produced by various manufacturers.  
There is a huge diversity in IoT device firmware, software stack and APIs offered for third party use. There is no reliable software support in form of firmware updates or security patches, for these devices.
The devices operate on limited hardware resources and stay online for several years after deployment. 
Given the heterogeneity of device types, functionalities and available resources, it is very challenging to develop generic endpoint security solutions for IoT devices, in particular, single-purpose IoT devices. 

\subsubsection*{\textbf{Complex Device Interactions}}

Network security solutions typically rely on traffic signatures to identify anomalies in the network~\cite{6517052, Feamster:2010:OHN:1851307.1851317}.
These solutions produce low false positives and work at line speeds.
However, given the numerous types of IoT devices and possible modes of interactions among these devices, it becomes practically infeasible to collect and maintain traffic signatures databases, used by signature-based network security solutions. Traditional mechanisms for learning attack signatures such as honeypots, do not scale for IoT ecosystem because of sheer diversity and number of devices~\cite{Yu:2015:HTF:2834050.2834095}. 
Therefore, it limits the application of these solutions to secure IoT and edge networks.   

\subsubsection*{\textbf{Monitoring Intranet traffic}}
Network security solutions are typically deployed at network periphery and filter any incoming and outgoing traffic. 
Any malicious traffic within the network goes undetected by these solutions, rendering them ineffective for detecting D2D attacks. 
Meanwhile, it is crucial to secure D2D communications in the network, to prevent scenarios where attacker connects to a network and compromises all devices connected to the network. 

\subsubsection*{\textbf{Resource Limitations}}
Network security solutions require specialized hardware and skilled professionals for deployment and maintenance. This incurs high costs, limiting the use of these solutions to secure edge networks~\cite{Sherry:2012:MMS:2377677.2377680}. 

On the other hand, the efficiency of endpoint security solutions is limited by the underlying resources available on host devices. Lack of software and hardware support makes it impossible to run these solutions on single purpose IoT devices. Meanwhile, high (power and CPU) resource footprint of endpoint security solutions limits their usability for securing high end devices such as smartphones etc. as well~\cite{isAntiVirusGood,Oliner:2013:CCE:2517351.2517354}.

\subsubsection*{\textbf{Delays in detecting attacks}}
Network and endpoint security solutions typically rely on a central entity to provide signature(s) for detecting malicious traffic or files. The process of collecting information from networks and devices, analyzing it to identify new attacks and generate corresponding signatures, is time consuming. With zero-day vulnerabilities and rapid evolution in attacks, it is not uncommon that attacks are only discovered long after attackers have infiltrated the system. 

\subsubsection*{\textbf{Lack of Collaboration among edge nodes}}
The devices running endpoint security solutions often perform some local analysis to detect any attacks. Although, the edge nodes (running the analysis) share analysis results with their cloud services, there is no mechanism available for edge nodes to share the results on local analysis among themselves. This lack of collaboration results in increasing the time required to detect attacks. On the contrary, if edge nodes can collaborate for detecting any attacks, it will reduce the time taken to detect and thwart targeted attacks such as, geofenced attacks.

\subsubsection*{\textbf{Lack of automation}}
Typical SOHO and small enterprise networks are setup using low-end, mid-range network gateways and routers. Due to poorly designed interfaces and lack of support for automated configuration, the networks are rarely configured by users~\cite{7980167, Feamster:2010:OHN:1851307.1851317, Hafeez:2016:STS:3010079.3012014}. As the number of connected devices increases over time, lack of adequate configuration results in exposing all connected devices to adversaries.

It is clear that having a dedicated administrator to handle network configuration and management tasks, is an unrealistic requirement, given millions of edge networks~\cite{Feamster:2010:OHN:1851307.1851317}. Therefore, gateways should support automation for easy and efficient network management. 

Based on this discussion, the basic set of requirements for a security solution addressing the challenges posed by IoT, can be summarized as,
\begin{itemize}
\item
It should be easy to deploy and operate with minimal manual effort needed. Meanwhile, it should be low cost with limited resource footprint.

\item
It should be monitor inter as well as intra-network communications to detect various (\classB and \classM) types of network traffic generated by devices

\item 
Traffic analysis should be performed close to edge networks to immediately block any attacks and share analysis results with peer nodes, in privacy preserving manner. 

\end{itemize}
